Breakup dynamics in primary jet atomization using mesh- and interface- refined Cahn-Hilliard Navier-Stokes

We present a technique to perform interface-resolved simulations of complex breakup dynamics in two-phase flows using the Cahn-Hilliard Navier-Stokes equations. The method dynamically decreases the interface thickness parameter in relevant regions and simultaneously increases local mesh resolution, preventing numerical artifacts. We perform a detailed numerical simulation of pulsed jet atomization that shows a complex cascade of break-up mechanisms involving sheet rupture and filament formation. To understand the effect of refinement on the breakup, we analyze the droplet size distribution. The proposed approach opens up resolved simulations for various multiphase flow phenomena.

==> Sections/DialationErosion.tex <==
The phases in CHNS is described by a continuous changing variable $\phi$ ranging from -1 to 1. In order to identify the key regions of interest such as ligaments, small droplets, we utilize the idea inspired from the image processing literature. ({\color{red}{ Should go in footnote - not working:}} We restrict our discussion to the constant refinement case. Although the central idea remains the same, the deployment on octrees mesh in distributed setting is much more involved and is deferred to the future algorithm publication.) We perform a series of following steps to achieve our goal:
\begin{enumerate}
    \item As a first step, we convert the image from continuous $\phi$ to a binary 0/1 representation $\phi_{BW}$ by thresholding it at a certain value ($\delta$).
    \begin{equation*}
\phi_{BW} = \begin{cases}
1 & \quad \phi \leq  \delta, \\
0 & \quad \phi > \delta.
\end{cases}
\end{equation*}
The value of $\delta$ is decided such that the immersed phase gets the value of 1 and the bulk phase gets 0. We put $\delta$ to be 0.8 or -0.8 depending on the value of immersed phase.
\item We then perform a series of erosion step to shrink the region of immersed ($\phi_{BW} = 1$) phase.
\item We then perform a series of dilation step to expand the region of $\phi_{BW}$. We note that we need to perform more dilation than erosion in order to incorporate for the shrinking of the interface encountered in the first step. In our experiments, we found that typically 3 -- 4 extra dilation is sufficient. 
\item As the final detection step we take the difference of the pixels after the dilation ($\phi_{BWd}$) and $\phi_{BW}$. The pixels which are marked as 1 in $\phi_{BW}$ and 0 on $\phi_{BWd}$ constitutes the region of interest.
\item As the final step, we decrease the Cahn in the regions identified in the previous step and refine the interface interface ($\phi = 0$) with the appropriate resolution.
\end{enumerate} 

We note that other ideas like connected component analysis can also be applied to achieve a similar task, but it has a higher computational cost -- specifically in distributed setting and cannot identify all the key features of interest.



==> pgflibraryqrr.shapes.openrectangle.code.tex <==
\let\pgf@sh@openrectangle@full\pgf@sh@bg@rectangle
\let\pgf@sh@openrectangle@\pgf@sh@openrectangle@full
\def\pgf@sh@openrectangle@e    {\pgfsetrectcap\pgfpathmoveto{\SE}\pgfpathlineto{\NE}}
\def\pgf@sh@openrectangle@n    {\pgfsetrectcap\pgfpathmoveto{\NW}\pgfpathlineto{\NE}}
\def\pgf@sh@openrectangle@w    {\pgfsetrectcap\pgfpathmoveto{\SW}\pgfpathlineto{\NW}}
\def\pgf@sh@openrectangle@s    {\pgfsetrectcap\pgfpathmoveto{\SW}\pgfpathlineto{\SE}}
\def\pgf@sh@openrectangle@en{\pgfsetrectcap\pgfpathmoveto{\SE}\pgfpathlineto{\NE}\pgfpathlineto{\NW}}
\def\pgf@sh@openrectangle@ew{\pgfsetrectcap\pgfpathmoveto{\NW}\pgfpathlineto{\SW}\pgfpathmoveto{\SE}\pgfpathlineto{\NE}}
\def\pgf@sh@openrectangle@es{\pgfsetrectcap\pgfpathmoveto{\SW}\pgfpathlineto{\SE}\pgfpathlineto{\NE}}
\def\pgf@sh@openrectangle@enw{\pgfsetbuttcap
  \pgfpathmoveto{\pgfpointadd{\SE}{\pgfpointscale{-1}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}}
  \pgfpathlineto{\NE}\pgfpathlineto{\NW}\pgfpathlineto{\pgfpointadd{\SW}{\pgfpointscale{-1}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}}}
\def\pgf@sh@openrectangle@ens{\pgfsetbuttcap
  \pgfpathmoveto{\pgfpointadd{\SW}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}}
  \pgfpathlineto{\SE}\pgfpathlineto{\NE}\pgfpathlineto{\pgfpointadd{\NW}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}}}
\def\pgf@sh@openrectangle@ews{\pgfsetbuttcap
  \pgfpathmoveto{\pgfpointadd{\NE}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}
  \pgfpathlineto{\SE}\pgfpathlineto{\SW}\pgfpathlineto{\pgfpointadd{\NW}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}}
\def\pgf@sh@openrectangle@nw{\pgfsetrectcap\pgfpathmoveto{\NE}\pgfpathlineto{\NW}\pgfpathlineto{\SW}}
\def\pgf@sh@openrectangle@ns{\pgfsetrectcap\pgfpathmoveto{\NE}\pgfpathlineto{\NW}\pgfpathmoveto{\SW}\pgfpathlineto{\SE}}
\def\pgf@sh@openrectangle@nws{\pgfsetbuttcap
  \pgfpathmoveto{\pgfpointadd{\NE}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}
  \pgfpathlineto{\NW}\pgfpathlineto{\SW}\pgfpathlineto{\pgfpointadd{\SE}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}}
\def\pgf@sh@openrectangle@ws{\pgfsetrectcap\pgfpathmoveto{\NW}\pgfpathlineto{\SW}\pgfpathlineto{\SE}}
\def\pgf@sh@openrectangle@bbg@e{\pgfsetcornersarced{\pgfpointorigin}\pgfpathrectanglecorners{\southwest}{\northeast}}
\let\pgf@sh@openrectangle@bbg@n\pgf@sh@openrectangle@bbg@e
\let\pgf@sh@openrectangle@bbg@s\pgf@sh@openrectangle@bbg@e
\let\pgf@sh@openrectangle@bbg@w\pgf@sh@openrectangle@bbg@e
\let\pgf@sh@openrectangle@bbg@ns\pgf@sh@openrectangle@bbg@e
\let\pgf@sh@openrectangle@bbg@ew\pgf@sh@openrectangle@bbg@e
\let\pgf@sh@openrectangle@bbg@full\pgf@sh@openrectangle@full
\let\pgf@sh@openrectangle@bbg@\pgf@sh@openrectangle@
\let\pgf@sh@openrectangle@bbg@enw\pgf@sh@openrectangle@enw
\let\pgf@sh@openrectangle@bbg@ens\pgf@sh@openrectangle@ens
\let\pgf@sh@openrectangle@bbg@ews\pgf@sh@openrectangle@ews
\let\pgf@sh@openrectangle@bbg@nws\pgf@sh@openrectangle@nws
\def\pgf@sh@openrectangle@bbg@en{%
  \pgfpathmoveto{\pgfpointadd{\SE}{\pgfpointscale{-1}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}}%
  \pgfpathlineto{\NE}%
  \pgfsetcornersarced{\pgfpointorigin}%
  \pgfpathlineto{\pgfpointadd{\NW}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}}%
  \pgfpathlineto{\southwest}}
\def\pgf@sh@openrectangle@bbg@nw{%
  \pgfpathmoveto{\pgfpointadd{\NE}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}%
  \pgfpathlineto{\NW}%
  \pgfsetcornersarced{\pgfpointorigin}%
  \pgfpathlineto{\pgfpointadd{\SW}{\pgfpointscale{-1}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}}%
  \pgfpathlineto{\southwest\pgf@ya\pgf@y\northeast\pgf@y\pgf@ya}}
\def\pgf@sh@openrectangle@bbg@ws{%
  \pgfpathmoveto{\pgfpointadd{\NW}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}%
  \pgfpathlineto{\SW}%
  \pgfsetcornersarced{\pgfpointorigin}%
  \pgfpathlineto{\pgfpointadd{\SE}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}%
  \pgfpathlineto{\northeast}}
\def\pgf@sh@openrectangle@bbg@es{%
  \pgfpathmoveto{\pgfpointadd{\SW}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}}%
  \pgfpathlineto{\SE}%
  \pgfsetcornersarced{\pgfpointorigin}%
  \pgfpathlineto{\pgfpointadd{\NE}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}%
  \pgfpathlineto{\southwest\pgf@xa\pgf@x\northeast\pgf@x\pgf@xa}}
\pgfset{open rectangle sides/.initial=ns, open rectangle fill/.initial=}
\pgfdeclareshape{open rectangle}{%
  \inheritsavedanchors[from=rectangle]
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}     \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{north west}\inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{north east}\inheritanchor[from=rectangle]{south east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}      \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{base}      \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{base west} \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{base east} \inheritanchor[from=rectangle]{mid east}
  \behindbackgroundpath{%
    \pgfkeysgetvalue{/pgf/open rectangle fill}\pgf@temp
    \ifx\pgf@temp\pgfutil@empty
    \else
      \pgfextract@process\SW{\pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}%
      \pgf@xa\pgf@x\pgf@ya\pgf@y
      \pgfextract@process\NE{\pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}}%
      \pgf@xb\pgf@x\pgf@yb\pgf@y
      \pgfextract@process\NW{\pgf@x\pgf@xa\pgf@y\pgf@yb}%
      \pgfextract@process\SE{\pgf@x\pgf@xb\pgf@y\pgf@ya}%
      \csname pgf@sh@openrectangle@bbg@\pgfkeysvalueof{/pgf/open rectangle sides}\endcsname
      \pgfsetfillcolor{\pgfkeysvalueof{/pgf/open rectangle fill}}%
      \pgfusepath{fill}
    \fi
  }%
  \backgroundpath{%
    \pgfextract@process\SW{\pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}%
    \pgf@xa\pgf@x\pgf@ya\pgf@y
    \pgfextract@process\NE{\pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}}%
    \pgf@xb\pgf@x\pgf@yb\pgf@y
    \pgfextract@process\NW{\pgf@x\pgf@xa\pgf@y\pgf@yb}%
    \pgfextract@process\SE{\pgf@x\pgf@xb\pgf@y\pgf@ya}%
    \csname pgf@sh@openrectangle@\pgfkeysvalueof{/pgf/open rectangle sides}\endcsname}}
\endinput


==> pgflibraryqrr.trans.code.tex <==
\def\pgftransformxmirror#1{
  \pgfmathparse{#1}%
  \ifpgfmathunitsdeclared
    \pgf@xa\pgfmathresult pt\relax
    \advance\pgf@xa2\relax
    \pgftransformcm{-1}{0}{0}{1}{\pgfqpoint{+\the\pgf@xa}{+0pt}}%
  \else
    \pgftransformmirror{\pgfqpointxy{\pgfmathresult}{0}}{\pgfpointadd{\pgfqpointxy{\pgfmathresult}{0}}{\pgfqpointxy{0}{1}}}%
  \fi
}
\def\pgftransformymirror#1{
  \pgfmathparse{#1}%
  \ifpgfmathunitsdeclared
    \pgf@ya\pgfmathresult pt\relax
    \advance\pgf@ya2\relax
    \pgftransformcm{1}{0}{0}{-1}{\pgfqpoint{+0pt}{+\the\pgf@ya}}%
  \else
    \edef\pgf@marshal{\noexpand\pgftransformmirror{\noexpand\pgfqpointxy{0}{\pgfmathresult}}%
                                                  {\noexpand\pgfpointadd{\noexpand\pgfqpointxy{0}{\pgfmathresult}}{\noexpand\pgfqpointxy{1}{0}}}}%
    \pgf@marshal
  \fi}
\def\pgftransformmirror#1#2{%
  \pgfextract@process\pgf@tempa{#1}%
  \pgfpointnormalised{\pgfpointdiff{\pgf@tempa}{#2}}%
  \pgf@xa=\pgf@sys@tonumber\pgf@y\pgf@x
  \pgf@xb=\pgf@sys@tonumber\pgf@x\pgf@x
  \pgf@yb=\pgf@sys@tonumber\pgf@y\pgf@y
  \multiply\pgf@xa2\relax
  \pgf@xc=-\pgf@yb\advance\pgf@xc\pgf@xb
  \pgf@yc=-\pgf@xb\advance\pgf@yc\pgf@yb
  \edef\pgf@temp{{\the\pgf@xc}{+\the\pgf@xa}{+\the\pgf@xa}{+\the\pgf@yc}}%
  \expandafter\pgf@transformcm\pgf@temp{\pgf@tempa}%
  \pgftransformshift{\pgfpointscale{-1}{\pgf@tempa}}%
}
\def\pgfqtransformmirror#1{%
  \pgfpointnormalised{#1}%
  \pgf@xa=\pgf@sys@tonumber\pgf@y\pgf@x
  \pgf@xb=\pgf@sys@tonumber\pgf@x\pgf@x
  \pgf@yb=\pgf@sys@tonumber\pgf@y\pgf@y
  \multiply\pgf@xa2\relax
  \pgf@xc=-\pgf@yb\advance\pgf@xc\pgf@xb
  \pgf@yc=-\pgf@xb\advance\pgf@yc\pgf@yb
  \edef\pgf@temp{{\the\pgf@xc}{+\the\pgf@xa}{+\the\pgf@xa}{+\the\pgf@yc}}%
  \expandafter\pgf@transformcm\pgf@temp{\pgfpointorigin}%
}
\endinput


==> pgflibraryshapes.qrr.roundedrectangle.code.tex <==
\input tikzlibraryshapes.qrr.roundedrectangle.code.tex
\endinput


==> tikzlibrarynode-families.code.tex <==
\let\tikz@lib@nf@textheight\relax
\let\tikz@lib@nf@textdepth\relax
\let\tikz@lib@nf@textwidth\relax
\tikzset{
  Minimum Width/.code={%
    \pgfutil@ifundefined{\pgfpictureid @#1@width}{}{%
      \tikzset{/tikz/minimum width/.expand twice=+\csname\pgfpictureid @#1@width\endcsname}%
    }%
    \tikz@addmode{\pgfmathsetlengthmacro\tikz@lib@nf@outerxsep{\pgfkeysvalueof{/pgf/outer xsep}}\global\let\tikz@lib@nf@outerxsep\tikz@lib@nf@outerxsep}%
    \tikzset{
      prefix after command={%
        \pgfextra
          \pgfinterruptpath
            \pgfsettransform{\csname pgf@sh@nt@\tikzlastnode\endcsname}%
            \pgfpointanchor{\tikzlastnode}{east}%
            \pgf@xa=\pgf@x \pgf@ya=\pgf@y
            \pgfpointanchor{\tikzlastnode}{west}%
            \advance\pgf@xa-\pgf@x
            \advance\pgf@ya-\pgf@y
            \pgfmathveclen@{\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgf@ya}%
            \pgf@x\pgfmathresult pt\relax
            \advance\pgf@x-\tikz@lib@nf@outerxsep
            \advance\pgf@x-\tikz@lib@nf@outerxsep
            \pgfutil@ifundefined{\pgfpictureid @#1@width}{%
              \expandafter\xdef\csname\pgfpictureid @#1@width\endcsname{\the\pgf@x}%
            }{%
              \expandafter\ifdim\csname\pgfpictureid @#1@width\endcsname<\pgf@x
                \expandafter\xdef\csname\pgfpictureid @#1@width\endcsname{\the\pgf@x}%
              \fi
            }%
            \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter
            \tikz@atend@picture\expandafter\expandafter\expandafter{\expandafter\tikz@atend@picture\expandafter\tikz@lib@nf@save\expandafter{\pgfpictureid}{#1}{width}{width}}
          \endpgfinterruptpath
        \endpgfextra
      }%
    }%
  },
  Minimum Height/.code={%
    \pgfutil@ifundefined{\pgfpictureid @#1@height}{}{%
      \tikzset{/tikz/minimum height/.expand twice=+\csname\pgfpictureid @#1@height\endcsname}%
    }%
    \tikz@addmode{\pgfmathsetlengthmacro\tikz@lib@nf@outerysep{\pgfkeysvalueof{/pgf/outer ysep}}\global\let\tikz@lib@nf@outerysep\tikz@lib@nf@outerysep}%
    \tikzset{
      prefix after command={%
        \pgfextra
          \pgfinterruptpath
            \pgfsettransform{\csname pgf@sh@nt@\tikzlastnode\endcsname}%
            \pgfpointanchor{\tikzlastnode}{north}%
            \pgf@xa=\pgf@x \pgf@ya=\pgf@y
            \pgfpointanchor{\tikzlastnode}{south}%
            \advance\pgf@xa-\pgf@x
            \advance\pgf@ya-\pgf@y
            \pgfmathveclen@{\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgf@ya}%
            \pgf@x\pgfmathresult pt\relax
            \advance\pgf@x-\tikz@lib@nf@outerysep
            \advance\pgf@x-\tikz@lib@nf@outerysep
            \pgfutil@ifundefined{\pgfpictureid @#1@height}{%
              \expandafter\xdef\csname\pgfpictureid @#1@height\endcsname{\the\pgf@x}%
            }{%
              \expandafter\ifdim\csname\pgfpictureid @#1@height\endcsname<\pgf@x
                \expandafter\xdef\csname\pgfpictureid @#1@height\endcsname{\the\pgf@x}%
              \fi
            }%
            \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter
            \tikz@atend@picture\expandafter\expandafter\expandafter{\expandafter\tikz@atend@picture\expandafter\tikz@lib@nf@save\expandafter{\pgfpictureid}{#1}{height}{height}}
          \endpgfinterruptpath
        \endpgfextra
      }%
    }%
  },
  Minimum Size/.style={
    Minimum Height={#1},
    Minimum Width={#1}},
  Text Height/.code=\edef\tikz@lib@nf@textheight{#1},
  Text Depth/.code= \edef\tikz@lib@nf@textdepth{#1},
  Text Width/.code=%
    \edef\tikz@lib@nf@textwidth{#1}%
    \pgfutil@ifundefined{\pgfpictureid @#1@textwidth}{}{%
      \tikzset{text width/.expand twice=+\csname\pgfpictureid @#1@textwidth\endcsname}%
    }%
}

\def\tikz@lib@nf@text@#1#2#3{%
  \expandafter\ifx\csname tikz@lib@nf@#3\endcsname\relax\else
    \ifx#1\wd\def\tikz@temp{@}\else\let\tikz@temp\pgfutil@empty\fi
    \expandafter\ifx\csname tikz@lib@nf@#3\tikz@temp\endcsname\pgfutil@empty\else
      \pgfutil@ifundefined{\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp}{%
        \expandafter\xdef\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp\endcsname{\the#1#2}%
      }{%
        \ifdim\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp\endcsname<#1#2
          \expandafter\xdef\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp\endcsname{\the#1#2}%
        \else
          \ifx#1\wd\else
            #1#2=\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\endcsname\relax
          \fi
        \fi
      }%
      \edef\tikz@temp{\noexpand\tikz@lib@nf@save{\pgfpictureid}{\csname tikz@lib@nf@#3\endcsname}{#3}{#3\tikz@temp}}%
      \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter
      \tikz@atend@picture\expandafter\expandafter\expandafter{\expandafter\tikz@atend@picture\tikz@temp}%
    \fi
  \fi
}
%%% Redefinition
\def\tikz@fig@continue{%
    \ifx\tikz@text@width\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@width}%
      \wd\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@height\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@height}%
      \ht\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@depth\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@depth}%
      \dp\pgfnodeparttextbox=\pgf@x%
    \fi%
    %
    %
    %
    \tikz@lib@nf@text@\ht\pgfnodeparttextbox{textheight}%
    \tikz@lib@nf@text@\dp\pgfnodeparttextbox{textdepth}%
    \tikz@lib@nf@text@\wd\pgfnodeparttextbox{textwidth}%
    %
    % Node transformation
    %
    \tikz@node@transformations
    %
    \setbox\tikz@figbox=\hbox{%
      \setbox\pgfutil@tempboxa=\copy\tikz@figbox%
      \unhbox\pgfutil@tempboxa%
      \hbox{{%
          \pgfinterruptpath%
            \pgfscope%
              \tikz@options%
              \setbox\tikz@figbox=\box\pgfutil@voidb@x%
              \pgfmultipartnode{\tikz@shape}{\tikz@anchor}{\tikz@fig@name}{%
                \pgfutil@tempdima=\pgflinewidth%
                {\begingroup\tikz@finish}%
                \global\pgflinewidth=\pgfutil@tempdima%
              }%
            \endpgfscope
          \endpgfinterruptpath%
      }}%
    }%
    %
    \tikz@alias%
    \tikz@node@finish%
}
\def\tikz@lib@nf@save#1#2#3#4{%
  \pgfutil@ifundefined{#1@#2@#3@done}{%
    \expandafter\let\csname#1@#2@#3@done\endcsname\pgfutil@empty%
    \immediate\write\pgfutil@auxout{\noexpand\expandafter\noexpand\gdef\noexpand\csname#1@#2@#3\endcsname{\csname#1@#2@#4\endcsname}}
  }{}%
}
\endinput


==> tikzlibrarynorm.code.tex <==
\tikzset{
	Norm/.code={%
		\pgfmathparse{#1}%
		\edef\qrr@tikz@norm{\pgfmathresult\ifpgfmathunitsdeclared pt\fi}%
		\let\ifqrr@tikz@normcs@unitsdeclared\ifpgfmathunitsdeclared},
	Norm=1,
	norm/.style={to path={-- ++(norm cs: \tikztotarget\space from \tikztostart) \tikztonodes}}
}
\newif\ifqrr@tikz@normcs@unitsdeclared
\newdimen\qrr@pgf@normcs@from@x\newdimen\qrr@pgf@normcs@from@y
\tikzdeclarecoordinatesystem{norm}{%
	\begingroup
		\let\qrr@next\relax
		\pgfutil@in@{ for }{#1}%
		\ifpgfutil@in@
			\qrr@tikz@normcs@parse@for#1\@qrr@tikz@normcs@parse@for
		\else
			\def\pgf@tempa{#1}%
		\fi
		\edef\pgf@marshal{\noexpand\pgfutil@in@{ from }{\pgf@tempa}}\pgf@marshal
		\ifpgfutil@in@
			\expandafter\qrr@tikz@normcs@parse@from\pgf@tempa\@qrr@tikz@normcs@parse@from
			\let\qrr@next\qrr@tikz@normcs@calc@hard
		\else
			\let\qrr@tikz@normcs@parse@to\pgf@tempa
			\qrr@pgf@normcs@from@x\z@
			\qrr@pgf@normcs@from@y\z@
		\fi
		\expandafter\qrr@tikz@normcs@parse@@to\expandafter{\qrr@tikz@normcs@parse@to}%
}
\def\qrr@tikz@normcs@calc@easy#1{%
	\pgf@xx\@ne
	\pgf@yy\@ne
	\pgf@xy\z@
	\pgf@yx\z@
	\tikz@scan@one@point\pgfutil@firstofone(#1)\relax
	\pgf@xa\pgf@x\pgf@ya\pgf@y
}
\def\qrr@tikz@normcs@calc@hard#1{%
	\tikz@scan@one@point\pgfutil@firstofone(#1)\relax
	\pgf@xa\pgf@x\pgf@ya\pgf@y
	\advance\pgf@xa-\qrr@pgf@normcs@from@x
	\advance\pgf@ya-\qrr@pgf@normcs@from@y
	\pgfpointnormalised{\pgfqpoint{\pgf@xa}{\pgf@ya}}
	\pgfmathsetlength\pgf@xa{\pgf@yy*\pgf@x-\pgf@yx*\pgf@y}
	\pgfmathsetlength\pgf@ya{-\pgf@xy*\pgf@x+\pgf@xx*\pgf@y}
}
\def\qrr@tikz@normcs@calc@unit#1{%
	\tikz@scan@one@point\pgfutil@firstofone(#1)\relax
	\pgf@xa\pgf@x\pgf@ya\pgf@y
	\advance\pgf@xa-\qrr@pgf@normcs@from@x
	\advance\pgf@ya-\qrr@pgf@normcs@from@y
	\pgfpointnormalised{\pgfqpoint{\pgf@xa}{\pgf@ya}}
	\pgf@xa\pgf@x\pgf@ya\pgf@y
}
\def\qrr@tikz@normcs@parse@@to#1{%
		\ifqrr@tikz@normcs@unitsdeclared
			\let\qrr@next\qrr@tikz@normcs@calc@unit
		\else
			\ifx\qrr@next\relax
			  \pgfutil@in@{cs:}{#1}%
			  \ifpgfutil@in@
			    \let\qrr@next\qrr@tikz@normcs@calc@hard
			  \else
			    \pgfutil@in@{intersection }{#1}%
			    \ifpgfutil@in@
			      \let\qrr@next\qrr@tikz@normcs@calc@hard
			    \else
			      \pgfutil@in@|{#1}%
			      \ifpgfutil@in@
			        \let\qrr@next\qrr@tikz@normcs@calc@hard
			      \else
			        \pgfutil@in@:{#1}%
			        \ifpgfutil@in@
			          \let\qrr@next\qrr@tikz@normcs@calc@easy
			        \else
			          \pgfutil@in@,{#1}%
			          \ifpgfutil@in@
			            \let\qrr@next\qrr@tikz@normcs@calc@easy
			          \else
			            \let\qrr@next\qrr@tikz@normcs@calc@hard
			          \fi
			        \fi
			      \fi
			    \fi
			  \fi
			\fi
		\fi
		\qrr@next{#1}%
		\pgfmathatantwo{+\pgf@xa}{+\pgf@ya}%
		\ifqrr@tikz@normcs@unitsdeclared
			\edef\pgf@marshal{\noexpand\pgfpointpolar{\pgfmathresult}{\qrr@tikz@norm}}
		\else
			\edef\pgf@marshal{\noexpand\pgfpointpolarxy{\pgfmathresult}{\qrr@tikz@norm}}
		\fi
		\pgfmath@smuggleone\pgf@marshal
	\endgroup
	\pgf@marshal

}

\def\qrr@tikz@normcs@parse@from#1 from #2\@qrr@tikz@normcs@parse@from{%
	\def\qrr@tikz@normcs@parse@to{#1}%
	\tikz@scan@one@point\pgfutil@firstofone(#2)\relax
	\qrr@pgf@normcs@from@x\pgf@x
	\qrr@pgf@normcs@from@y\pgf@y
}
\def\qrr@tikz@normcs@parse@for#1 for #2\@qrr@tikz@normcs@parse@for{%
	\def\pgf@tempa{#1}%
	\pgfkeysalso{/tikz/Norm={#2}}%
}

% a fix for the 2.10 version of PGF/TikZ
\expandafter\let\expandafter\pgfmathatantwo\csname pgfmathatan2\endcsname


==> tikzlibrarypaths.ortho.code.tex <==
\let\tikz@orig@rect\tikz@rect
\def\tikz@rect{\pgfutil@ifnextchar e\tikz@orig@rect\qrr@tikz@r}
\def\qrr@tikz@r -{%
  \pgfutil@ifnextchar l\qrr@tikz@lr@lineto{%
    \pgfutil@ifnextchar r\qrr@tikz@rl@lineto{%
      \pgfutil@ifnextchar u\qrr@tikz@ud@lineto{%
        \pgfutil@ifnextchar d\qrr@tikz@du@lineto\tikz@expand
      }%
    }%
  }%
}
\let\tikz@orig@vh@lineto@next\tikz@vh@lineto@next
\def\tikz@vh@lineto@next{%
  \pgfutil@ifnextchar|{\expandafter\qrr@tikz@vhv@lineto\pgfutil@gobble}%
    {\pgfutil@ifnextchar\tikz@activebar{\expandafter\qrr@tikz@vhv@lineto\pgfutil@gobble}%
      {\tikz@orig@vh@lineto@next}}}
\let\tikz@orig@hv@lineto\tikz@hv@lineto
\def\tikz@hv@lineto{%
  \pgfutil@ifnextchar-{\expandafter\qrr@tikz@hvh@lineto\pgfutil@gobble}%
    {\tikz@orig@hv@lineto}}
\tikzset{%
  |-|/.style={%
   /utils/exec=\pgfmathsetmacro\qrr@tikz@hvvh@ratio{#1},%
   to path={|-| (\tikztotarget) \tikztonodes}},%
  -|-/.style={%
   /utils/exec=\pgfmathsetmacro\qrr@tikz@hvvh@ratio{#1},%
   to path={-|- (\tikztotarget) \tikztonodes}},%
  ud/.style={%
    udlr/ud distance/.expanded={#1},%
    to path={r-ud (\tikztotarget) \tikztonodes}},%
  du/.style={%
    udlr/du distance/.expanded={#1},%
    to path={r-du (\tikztotarget) \tikztonodes}},%
  lr/.style={%
    udlr/lr distance/.expanded={#1},%
    to path={r-lr (\tikztotarget) \tikztonodes}},%
  rl/.style={%
    udlr/rl distance/.expanded={#1},%
    to path={r-rl (\tikztotarget) \tikztonodes}},%
  ud/.default=\pgfkeysvalueof{/tikz/udlr/ud distance},%
  du/.default=\pgfkeysvalueof{/tikz/udlr/du distance},%
  rl/.default=\pgfkeysvalueof{/tikz/udlr/rl distance},%
  lr/.default=\pgfkeysvalueof{/tikz/udlr/lr distance},%
  |-|/.default=\qrr@tikz@hvvh@ratio,%
  -|-/.default=\qrr@tikz@hvvh@ratio
}

%BEGIN_FOLD hvvh operator
\def\qrr@tikz@vhv@lineto{\pgfutil@ifnextchar[{\qrr@tikz@collect@hvvh@options\qrr@tikz@vhv@lineto@next}{\qrr@tikz@collect@hvvh@options\qrr@tikz@vhv@lineto@next[]}}
\def\qrr@tikz@hvh@lineto{\pgfutil@ifnextchar[{\qrr@tikz@collect@hvvh@options\qrr@tikz@hvh@lineto@next}{\qrr@tikz@collect@hvvh@options\qrr@tikz@hvh@lineto@next[]}}
%END_FOLD

%BEGIN_FOLD udlr operators
%% ud style
\def\qrr@tikz@rl@lineto rl{\pgfutil@ifnextchar[{\qrr@tikz@collect@hvvh@options\qrr@tikz@rl@lineto@next}{\qrr@tikz@collect@hvvh@options\qrr@tikz@rl@lineto@next[]}}
\def\qrr@tikz@lr@lineto lr{\pgfutil@ifnextchar[{\qrr@tikz@collect@hvvh@options\qrr@tikz@lr@lineto@next}{\qrr@tikz@collect@hvvh@options\qrr@tikz@lr@lineto@next[]}}
\def\qrr@tikz@du@lineto du{\pgfutil@ifnextchar[{\qrr@tikz@collect@hvvh@options\qrr@tikz@du@lineto@next}{\qrr@tikz@collect@hvvh@options\qrr@tikz@du@lineto@next[]}}
\def\qrr@tikz@ud@lineto ud{\pgfutil@ifnextchar[{\qrr@tikz@collect@hvvh@options\qrr@tikz@ud@lineto@next}{\qrr@tikz@collect@hvvh@options\qrr@tikz@ud@lineto@next[]}}
%END_FOLD

\input tikzlibrarypaths.ortho.tex
\endinput


==> tikzlibrarypaths.ortho.tex <==
\newlength\qrr@tikz@udlr@distance
\newlength\qrr@tikz@hvvh@distance
\newif\ifqrr@tikz@hvvh@middle
\newif\ifqrr@tikz@hvvh@fromcenter
\newif\iftikz@ortho@preflush
\tikz@ortho@preflushtrue
\let\tikz@origtotarget\pgfutil@empty

%%% |-/-|
\tikzset{
  |-/.style={to path={|- (\tikztotarget) \tikztonodes}},
  -|/.style={to path={-| (\tikztotarget) \tikztonodes}},
  *|/.style={to path={%
    \pgfextra
      \iftikz@shapeborder
        \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
        \ifdim\pgf@y>\tikz@lasty\relax
          \edef\tikztostart{\tikztostart.north}%
        \else
          \edef\tikztostart{\tikztostart.south}%
        \fi
      \fi
    \endpgfextra
    (perpendicular cs: horizontal line through={(\tikztostart)},
                       vertical line through={(\tikztotarget)}) -- (\tikztotarget) \tikztonodes
  }},
  *-/.style={to path={%
    \pgfextra
      \iftikz@shapeborder
        \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
        \ifdim\pgf@x>\tikz@lastx\relax
          \edef\tikztostart{\tikztostart.east}%
        \else
          \edef\tikztostart{\tikztostart.west}%
        \fi
      \fi
    \endpgfextra
    (perpendicular cs: vertical line through={(\tikztostart)},
                     horizontal line through={(\tikztotarget)}) -- (\tikztotarget) \tikztonodes
  }},
  |*/.style={to path={%
    \pgfextra
      \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
      \iftikz@shapeborder
        \let\tikz@origtotarget\tikztotarget
        \ifdim\pgf@y>\tikz@lasty\relax
          \edef\tikztotarget{\tikztotarget.south}%
        \else
          \edef\tikztotarget{\tikztotarget.north}%
        \fi
      \fi
    \endpgfextra
    (\tikztostart) -- (perpendicular cs: vertical line through={(\tikztostart)},
                                         horizontal line through={(\tikztotarget)})
    \tikztonodes \ifx\tikz@origtotarget\pgfutil@empty\else\iftikz@ortho@preflush(\tikz@origtotarget)\fi\fi
  }},
  -*/.style={to path={%
    \pgfextra
      \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
      \iftikz@shapeborder
        \let\tikz@origtotarget\tikztotarget
        \ifdim\pgf@x>\tikz@lastx\relax
          \edef\tikztotarget{\tikztotarget.west}%
        \else
          \edef\tikztotarget{\tikztotarget.east}%
        \fi
      \fi
    \endpgfextra
    (\tikztostart) -- (perpendicular cs: horizontal line through={(\tikztostart)},
                                         vertical line through={(\tikztotarget)})
    \tikztonodes \ifx\tikz@origtotarget\pgfutil@empty\else\iftikz@ortho@preflush(\tikz@origtotarget)\fi\fi
  }},
  node as new start/.is if=tikz@ortho@preflush
}

%%% HVVH/UDLR
\tikzset{
  hvvh/.code={\pgfqkeys{/tikz/hvvh}{#1}},%
  udlr/.code={\pgfqkeys{/tikz/udlr}{#1}},%
%  hvvh/.search also=/tikz/udlr,%
  udlr/.search also=/tikz/hvvh,% endless loop?
  hvvh/middle 0 to 1/.style={hvvh/spacing=0},%
  hvvh/0 to 1/.style={hvvh/middle 0 to 1},%
  hvvh/from center/.is if=qrr@tikz@hvvh@fromcenter,%
  udlr/from center/.style={/tikz/hvvh/from center={#1}},
  udlr/from center/.default=true,
  hvvh/spacing/.code=%
    \ifcase#1\relax
      \qrr@tikz@hvvh@middletrue
      \def\qrr@tikz@hvvh@timing@parts{1}%
      \def\qrr@tikz@hvvh@timing@first{0}%
      \def\qrr@tikz@hvvh@timing@last{1}%
      \def\qrr@tikz@hvvh@timing@subtr{0}%
      \def\qrr@tikz@hvvh@timing@factor{1}%
    \else
      \qrr@tikz@hvvh@middlefalse
      \def\qrr@tikz@hvvh@timing@parts{#1}%
      \pgfmathreciprocal{#1}\let\qrr@tikz@hvvh@timing@first\pgfmathresult
      \pgfmathsetmacro\qrr@tikz@hvvh@timing@last{1-\pgfmathresult}%
      \pgfmathreciprocal{#1-2}%
      \let\qrr@tikz@hvvh@timing@subtr\pgfmathresult
      \pgfmathsetmacro\qrr@tikz@hvvh@timing@factor{1+2*\pgfmathresult}%
    \fi,
  hvvh/ratio/.code=\pgfmathsetmacro\qrr@tikz@hvvh@ratio{#1},
  hvvh/distance/.code=\pgfmathsetlength\qrr@tikz@hvvh@distance{#1}\let\qrr@tikz@hvvh@ratio\pgfutil@empty,%
  udlr/distance/.style={/tikz/udlr/ud distance={#1},/tikz/udlr/du distance={#1},/tikz/udlr/lr distance={#1},/tikz/udlr/rl distance={#1}},%
  udlr/ud distance/.initial=+.5cm,%
  udlr/du distance/.initial=+.5cm,%
  udlr/lr distance/.initial=+.5cm,%
  udlr/rl distance/.initial=+.5cm%
}
\tikzset{% default
  hvvh/ratio=.5,%
  hvvh/spacing=4%
}

%BEGIN_FOLD Timer
\def\tikz@timer@hvhline{%
  \pgf@process{\tikz@timer@start}\pgf@ya\pgf@y
  \pgf@process{\tikz@timer@end}\pgf@yc\pgf@y
  \pgf@process{\tikz@timer@middle}\pgf@xb\tikz@time pt%
  \ifdim\tikz@time pt<\qrr@tikz@hvvh@timing@first pt% first quarter
    \ifqrr@tikz@hvvh@middle
      \advance\pgf@xb1pt%
    \else
      \pgf@xb\qrr@tikz@hvvh@timing@parts\pgf@xb
    \fi
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}{\noexpand\tikz@timer@start}{%
        \noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@ya}}}%
  \else
    \ifdim\tikz@time pt>\qrr@tikz@hvvh@timing@last pt% last quarter
      \ifqrr@tikz@hvvh@middle
        \advance\pgf@xb-1pt%
      \else
        \pgf@xb\qrr@tikz@hvvh@timing@parts\pgf@xb
      \fi
      \advance\pgf@xb\dimexpr-\qrr@tikz@hvvh@timing@parts pt+1pt\relax%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@yc}}{\noexpand\tikz@timer@end}}%
    \else% middle half
      \pgf@xb\qrr@tikz@hvvh@timing@factor\pgf@xb%
      \advance\pgf@xb-\qrr@tikz@hvvh@timing@subtr pt%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@ya}}{\noexpand\tikz@timer@middle}}%
    \fi\fi\tikz@marshal}
\def\tikz@timer@vhvline{%
  \pgf@process{\tikz@timer@start}\pgf@xa\pgf@x
  \pgf@process{\tikz@timer@end}\pgf@xc\pgf@x
  \pgf@process{\tikz@timer@middle}\pgf@xb\tikz@time pt%
  \ifdim\tikz@time pt<\qrr@tikz@hvvh@timing@first pt% first quarter
    \ifqrr@tikz@hvvh@middle
      \advance\pgf@xb1pt%
    \else
      \pgf@xb\qrr@tikz@hvvh@timing@parts\pgf@xb
    \fi
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}{\noexpand\tikz@timer@start}{%
        \noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@y}}}%
  \else
    \ifdim\tikz@time pt>\qrr@tikz@hvvh@timing@last pt% last quarter
    \ifqrr@tikz@hvvh@middle
      \advance\pgf@xb-1pt%
    \else
      \pgf@xb\qrr@tikz@hvvh@timing@parts\pgf@xb
    \fi
      \advance\pgf@xb by\dimexpr-\qrr@tikz@hvvh@timing@parts pt+1pt\relax%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@y}}{\noexpand\tikz@timer@end}}%
    \else% middle half
      \pgf@xb=\qrr@tikz@hvvh@timing@factor\pgf@xb
      \advance\pgf@xb by-\qrr@tikz@hvvh@timing@subtr pt%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@y}}{\noexpand\tikz@timer@middle}}%
      \fi\fi\tikz@marshal}

%END_FOLD
\let\tikz@hvvh@currentoption\pgfutil@empty
\def\qrr@tikz@collect@hvvh@options#1[#2]{\edef\tikz@hvvh@currentoption{#2}#1}
\def\qrr@tikz@hvh@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\qrr@tikz@hvh@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\qrr@tikz@hvh@lineto@next}%
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\qrr@tikz@hvh@lineto@next}{\tikz@scan@one@point\qrr@tikz@@hvh@lineto}}}}
\def\qrr@tikz@vhv@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\qrr@tikz@vhv@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\qrr@tikz@vhv@lineto@next}%
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\qrr@tikz@vhv@lineto@next}{\tikz@scan@one@point\qrr@tikz@@vhv@lineto}}}}
\def\qrr@tikz@ud@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\qrr@tikz@ud@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\qrr@tikz@ud@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\qrr@tikz@ud@lineto@next}{\tikz@scan@one@point\qrr@tikz@@ud@lineto}}}}
\def\qrr@tikz@du@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\qrr@tikz@du@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\qrr@tikz@du@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\qrr@tikz@du@lineto@next}{\tikz@scan@one@point\qrr@tikz@@du@lineto}}}}
\def\qrr@tikz@lr@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\qrr@tikz@lr@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\qrr@tikz@lr@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\qrr@tikz@lr@lineto@next}{\tikz@scan@one@point\qrr@tikz@@lr@lineto}}}}
\def\qrr@tikz@rl@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\qrr@tikz@rl@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\qrr@tikz@rl@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\qrr@tikz@rl@lineto@next}{\tikz@scan@one@point\qrr@tikz@@rl@lineto}}}}

\def\tikz@do@hvvh#1#2#3#4#5{%
% #1 = first kink
% #2 = second kink
% #3 = end
% #4 = timer
% #5 = tikz@shapeborder@name
  \pgfpathlineto{#1}%
  \pgfpathlineto{#2}%
  \pgfpathlineto{#3}%
  \def\tikz@timer@middle{#2}%
  \def\tikz@timer@end{#3}%
  \let\tikz@timer#4
  \edef\pgf@temp{#5}%
  \ifx\pgf@temp\pgfutil@empty
    \let\tikz@moveto@waiting\relax
  \else
    \edef\tikz@moveto@waiting{#5}%
  \fi
  \tikz@scan@next@command%
}
%BEGIN_FOLD hvvh operator
%% -|- operator
\def\qrr@tikz@@hvh@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xb=\tikz@lastx
  \pgf@xc=\tikz@lastx
  \pgf@yc=\tikz@lasty
  \tikz@make@last@position{#1}%
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\pgf@yc}}\pgf@xc\pgf@yc
  \begingroup
    \pgfqkeys{/tikz/hvvh}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \iftikz@shapeborder
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@xb}{\tikz@lasty}}}%
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \fi
      \ifx\qrr@tikz@hvvh@ratio\pgfutil@empty
        \ifdim\qrr@tikz@hvvh@distance<0pt\relax
          \ifqrr@tikz@hvvh@fromcenter
            \pgf@xc\tikz@lastx
          \else
            \pgf@xc\pgf@x
          \fi
        \fi
        \ifdim\pgf@x>\tikz@lastx
          \qrr@tikz@hvvh@distance-\qrr@tikz@hvvh@distance
        \fi
      \else
        \ifqrr@tikz@hvvh@fromcenter
          \qrr@tikz@hvvh@distance\tikz@lastx
        \else
          \qrr@tikz@hvvh@distance\pgf@x
        \fi
        \advance\qrr@tikz@hvvh@distance-\pgf@xc
        \qrr@tikz@hvvh@distance\qrr@tikz@hvvh@ratio\qrr@tikz@hvvh@distance
      \fi
      \advance\pgf@xc\qrr@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
      \edef\pgf@temp{\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \fi
      \ifx\qrr@tikz@hvvh@ratio\pgfutil@empty
        \ifdim\qrr@tikz@hvvh@distance<0pt\relax
          \pgf@xc\tikz@lastx
        \fi
        \ifdim\pgf@x>\tikz@lastx
          \qrr@tikz@hvvh@distance-\qrr@tikz@hvvh@distance
        \fi
      \else
        \qrr@tikz@hvvh@distance\tikz@lastx
        \advance\qrr@tikz@hvvh@distance-\pgf@xc
        \qrr@tikz@hvvh@distance\qrr@tikz@hvvh@ratio\qrr@tikz@hvvh@distance
      \fi
      \advance\pgf@xc\qrr@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
      \edef\pgf@temp{\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi%
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\expandafter\noexpand\pgf@tempa}%
        {\expandafter\noexpand\pgf@tempb}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@hvhline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}

%% |-| operator
\def\qrr@tikz@@vhv@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc=\tikz@lastx
  \pgf@yb=\tikz@lasty
  \pgf@yc=\tikz@lasty
  \tikz@make@last@position{#1}%
  \tikz@flush@moveto@toward{\pgfqpoint{\pgf@xc}{\tikz@lasty}}\pgf@xc\pgf@yc
  \begingroup
    \pgfqkeys{/tikz/hvvh}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \iftikz@shapeborder
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\tikz@lastx}{\pgf@yb}}}%
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \fi
      \ifx\qrr@tikz@hvvh@ratio\pgfutil@empty
        \ifdim\qrr@tikz@hvvh@distance<0pt\relax
          \ifqrr@tikz@hvvh@fromcenter
            \pgf@yc\tikz@lasty
          \else
            \pgf@yc\pgf@y
          \fi
        \fi
        \ifdim\pgf@y>\tikz@lasty
          \qrr@tikz@hvvh@distance-\qrr@tikz@hvvh@distance
        \fi
      \else
        \ifqrr@tikz@hvvh@fromcenter
          \qrr@tikz@hvvh@distance\tikz@lasty
        \else
          \qrr@tikz@hvvh@distance\pgf@y
        \fi
        \advance\qrr@tikz@hvvh@distance-\pgf@yc
        \qrr@tikz@hvvh@distance\qrr@tikz@hvvh@ratio\qrr@tikz@hvvh@distance
      \fi
      \advance\pgf@yc\qrr@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
      \edef\pgf@temp{\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \fi
      \ifx\qrr@tikz@hvvh@ratio\pgfutil@empty
        \ifdim\qrr@tikz@hvvh@distance<0pt\relax
          \pgf@yc\tikz@lasty
        \fi
        \ifdim\pgf@y>\tikz@lasty
          \qrr@tikz@hvvh@distance-\qrr@tikz@hvvh@distance
        \fi
      \else
        \qrr@tikz@hvvh@distance\tikz@lasty
        \advance\qrr@tikz@hvvh@distance-\pgf@yc
        \qrr@tikz@hvvh@distance\qrr@tikz@hvvh@ratio\qrr@tikz@hvvh@distance
      \fi
      \advance\pgf@yc\qrr@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
      \edef\pgf@temp{\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi%
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\expandafter\noexpand\pgf@tempa}%
        {\expandafter\noexpand\pgf@tempb}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@vhvline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}

%% ud operator
\def\qrr@tikz@@ud@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc\tikz@lastx
  \pgf@yb\tikz@lasty
  \advance\tikz@lasty1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/udlr}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\qrr@tikz@udlr@distance{\pgfkeysvalueof{/tikz/udlr/ud distance}}%
    \iftikz@shapeborder
      \advance\pgf@y1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \else\ifx\pgf@temp\relax
          \pgf@yc\pgf@yb
        \fi
      \fi
      \ifdim\pgf@yc<\pgf@y
        \ifqrr@tikz@hvvh@fromcenter
          \pgf@yc=\tikz@lasty
        \else
          \pgf@yc=\pgf@y
        \fi
      \fi
      \advance\pgf@yc\qrr@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifx\pgf@temp\relax\else
        \ifqrr@tikz@hvvh@fromcenter\else
          \pgf@yb\pgf@yc
        \fi
      \fi
      \ifdim\pgf@yb<\tikz@lasty\pgf@yb\tikz@lasty\fi
      \advance\pgf@yb\qrr@tikz@udlr@distance
      \pgf@yc\pgf@yb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@vhvline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}

%% du operator
\def\qrr@tikz@@du@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc\tikz@lastx
  \pgf@yb\tikz@lasty
  \advance\tikz@lasty-1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/udlr}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\qrr@tikz@udlr@distance{\pgfkeysvalueof{/tikz/udlr/du distance}}%
    \iftikz@shapeborder
      \advance\pgf@y-1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \else\ifx\pgf@temp\relax
          \pgf@yc\pgf@yb
        \fi
      \fi
      \ifdim\pgf@yc>\pgf@y
        \ifqrr@tikz@hvvh@fromcenter
          \pgf@yc=\tikz@lasty
        \else
          \pgf@yc=\pgf@y
        \fi
      \fi
      \advance\pgf@yc-\qrr@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifx\pgf@temp\relax\else
        \ifqrr@tikz@hvvh@fromcenter\else
          \pgf@yb\pgf@yc
        \fi
      \fi
      \ifdim\pgf@yb>\tikz@lasty\pgf@yb\tikz@lasty\fi
      \advance\pgf@yb-\qrr@tikz@udlr@distance
      \pgf@yc\pgf@yb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@vhvline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}

%% lr operator
\def\qrr@tikz@@lr@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xb\tikz@lastx
  \pgf@yc\tikz@lasty
  \advance\tikz@lastx-1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/udlr}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\qrr@tikz@udlr@distance{\pgfkeysvalueof{/tikz/udlr/lr distance}}%
    \iftikz@shapeborder
      \advance\pgf@x-1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \else\ifx\pgf@temp\relax
          \pgf@xc\pgf@xb
        \fi
      \fi
      \ifdim\pgf@xc>\pgf@x
        \ifqrr@tikz@hvvh@fromcenter
          \pgf@xc=\tikz@lastx
        \else
          \pgf@xc=\pgf@x
        \fi
      \fi
      \advance\pgf@xc-\qrr@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifx\pgf@temp\relax\else
        \ifqrr@tikz@hvvh@fromcenter\else
          \pgf@xb\pgf@xc
        \fi
      \fi
      \ifdim\pgf@xb>\tikz@lastx\pgf@xb\tikz@lastx\fi
      \advance\pgf@xb-\qrr@tikz@udlr@distance
      \pgf@xc\pgf@xb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@hvhline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}

%% rl operator
\def\qrr@tikz@@rl@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xb\tikz@lastx
  \pgf@yc\tikz@lasty
  \advance\tikz@lastx1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/udlr}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\qrr@tikz@udlr@distance{\pgfkeysvalueof{/tikz/udlr/rl distance}}%
    \iftikz@shapeborder%
      \advance\pgf@x1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \else\ifx\pgf@temp\relax
          \pgf@xc\pgf@xb
        \fi
      \fi
      \ifdim\pgf@xc<\pgf@x
        \ifqrr@tikz@hvvh@fromcenter
          \pgf@xc=\tikz@lastx
        \else
          \pgf@xc=\pgf@x
        \fi
      \fi
      \advance\pgf@xc\qrr@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty%
      \ifx\pgf@temp\relax\else
        \ifqrr@tikz@hvvh@fromcenter\else
          \pgf@xb\pgf@xc
        \fi
      \fi
      \ifdim\pgf@xb<\tikz@lastx\pgf@xb\tikz@lastx\fi
      \advance\pgf@xb\qrr@tikz@udlr@distance
      \pgf@xc\pgf@xb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@hvhline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}
%END_FOLD
\endinput


==> tikzlibrarypaths.rectangle.code.tex <==
% This is the TikZ library paths.rectangle
% Load with \usetikzlibrary{paths.rectangle}
%
% This small library extends the node placing algorithm (a.k.a. timer)
% so that nodes can be placed on the path of an rectangle.
%
% Styles are:
%  - rectangle original timer
%    The original placement between position 0 and 1 are not changed.
%    The rectangle's path can be accessed by positions between 1 and 2.
%  - rectangle new timer
%    This style switches the positions between 0 and 1 with those
%    between 1 and 2.

\def\qrr@tikz@timer@rect@origline{%
  \ifdim\tikz@time pt>1pt
    \pgfutil@tempdima\tikz@time pt
    \ifdim\pgfutil@tempdima<1.5pt
      \advance\pgfutil@tempdima-1pt
    \else
      \advance\pgfutil@tempdima-1.5pt
      \let\pgf@tempa\tikz@timer@start
      \let\tikz@timer@start\tikz@timer@end
      \let\tikz@timer@end\pgf@tempa
    \fi
    \multiply\pgfutil@tempdima2
    \edef\tikz@time{\strip@pt\pgfutil@tempdima}%
    \expandafter\tikz@timer@vhline
  \else\expandafter\tikz@timer@line\fi
}
\def\qrr@tikz@timer@rect@lineafterone{%
  \pgfutil@tempdima\tikz@time pt
  \ifdim\pgfutil@tempdima<1pt
    \ifdim\pgfutil@tempdima<.5pt\else
      \advance\pgfutil@tempdima-.5pt
      \let\pgf@tempa\tikz@timer@start
      \let\tikz@timer@start\tikz@timer@end
      \let\tikz@timer@end\pgf@tempa
    \fi
    \multiply\pgfutil@tempdima2
    \edef\tikz@time{\strip@pt\pgfutil@tempdima}%
    \expandafter\tikz@timer@vhline
  \else
    \advance\pgfutil@tempdima-1pt
    \edef\tikz@time{\strip@pt\pgfutil@tempdima}%
    \expandafter\tikz@timer@line
  \fi
}
\tikzset{
  rectangle original timer/.code=\let\tikz@timer@line\qrr@tikz@timer@rect@origline,
  rectangle new timer/.code=\let\tikz@timer@line\qrr@tikz@timer@rect@lineafterone,
  rectangle original timer
}


==> tikzlibrarypatterns.images.code.tex <==
% This is the TikZ library patterns.images
% Load with \usetikzlibrary{patterns.images}
%
% Macro:
%  - \pgfSetupImageAsPattern[<opt arguments for \pgfdeclareimage>]{<name>}{<path/file>}
%
% Keys are:
%  - use image as pattern=<name>
%  - image as pattern=<opt arguments for \pgftext>

\newlength\qrr@pgf@iap@width
\newlength\qrr@pgf@iap@height

\def\pgfSetupImageAsPattern{\pgfutil@ifnextchar[\qrr@pgfSetupImageAsPattern{\qrr@pgfSetupImageAsPattern[]}}
\def\qrr@pgfSetupImageAsPattern[#1]#2#3{% #1 = options
                                        % #2 = image name
                                        % #3 = file name
  \pgfdeclareimage[#1]{qrr@pgf@iap@#2}{#3}%
  \sbox\pgfutil@tempboxa{\pgfuseimage{qrr@pgf@iap@#2}}%
  \expandafter\edef\csname qrr@pgf@iap@#2@width\endcsname{\the\wd\pgfutil@tempboxa}%
  \expandafter\edef\csname qrr@pgf@iap@#2@height\endcsname{\the\ht\pgfutil@tempboxa}%
}
\tikzset{
  image as pattern/.code={
    \edef\qrr@pgf@iap@options{#1}%
    \pgfkeysalso{/tikz/path picture={%
      \pgf@process{\pgfpointanchor{path picture bounding box}{north east}}%
      \pgf@xa\pgf@x\pgf@ya\pgf@y
      \pgf@process{\pgfpointanchor{path picture bounding box}{south west}}%
      \pgf@xb\pgf@x\pgf@yb\pgf@y\pgf@yc\pgf@yb
      \pgfutil@loop
        {%
        \pgfutil@loop
          \expandafter\pgftext\expandafter[\qrr@pgf@iap@options,at=\pgfqpoint{\pgf@xb}{\pgf@yb}]{\pgfuseimage{qrr@pgf@iap@\qrr@pgf@iap@name}}%
          \ifdim\pgf@yb<\pgf@ya
          \advance\pgf@yb\qrr@pgf@iap@height
        \pgfutil@repeat
        }%
        \ifdim\pgf@xb<\pgf@xa
        \advance\pgf@xb\qrr@pgf@iap@width
        \pgf@yb\pgf@yc
      \pgfutil@repeat
    }}%
  },
  use image as pattern/.code={%
    \edef\qrr@pgf@iap@name{#1}%
    \expandafter\qrr@pgf@iap@width\csname qrr@pgf@iap@#1@width\endcsname
    \expandafter\qrr@pgf@iap@height\csname qrr@pgf@iap@#1@height\endcsname
  }
}
\endinput


==> tikzlibrarypositioning-plus.code.tex <==
% This is the TikZ library positioning-plus
% Load with \usetikzlibrary{positioning-plus}
%
% This small library extends TikZ options like 'above', 'left' or 'below right'
% so that they can be used with an optional prefixed factor seperated by ':' (colon)
%
% The option 'left=.5:of somenode' will place
% a new node .5cm (default 'node distance' is '1cm and 1cm') left to (somenode).
% The option 'above right=.2 and .7:of someothernode' will place
% a new node .2cm above and .7cm right of (someothernode).
%
% Additional the options 'xshift*' and 'yshift*' add an additional shift
% as a factor of 'node distance'
% Inspired by http://tex.stackexchange.com/a/117610/16595

\usetikzlibrary{positioning}
\usetikzlibrary{fit}

\pgfdeclaregenericanchor{corner south east}{%
  \pgf@sh@reanchor{#1}{south}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{east}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner north east}{%
  \pgf@sh@reanchor{#1}{north}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{east}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner south west}{%
  \pgf@sh@reanchor{#1}{south}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{west}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner north west}{%
  \pgf@sh@reanchor{#1}{north}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{west}}%
  \pgf@y\pgf@ya
}

\tikzset{corner above left/.code=\tikz@lib@place@handle@{#1}{corner south east}{-1}{1}{corner north west}{0.707106781}}
\tikzset{corner above right/.code=\tikz@lib@place@handle@{#1}{corner south west}{1}{1}{corner north east}{0.707106781}}
\tikzset{corner below left/.code=\tikz@lib@place@handle@{#1}{corner north east}{-1}{-1}{corner south west}{0.707106781}}
\tikzset{corner below right/.code=\tikz@lib@place@handle@{#1}{corner north west}{1}{-1}{corner south east}{0.707106781}}

\tikzset{corner north left/.code =\tikz@lib@place@handle@{#1}{corner north east}{-1}{0}{corner north west}{1}}
\tikzset{corner north right/.code=\tikz@lib@place@handle@{#1}{corner north west}{1}{0}{corner north east}{1}}
\tikzset{corner south left/.code =\tikz@lib@place@handle@{#1}{corner south east}{-1}{0}{corner south west}{1}}
\tikzset{corner south right/.code=\tikz@lib@place@handle@{#1}{corner south west}{1}{0}{corner south east}{1}}

\tikzset{corner west above/.code =\tikz@lib@place@handle@{#1}{corner south west}{0}{1}{corner north west}{1}}
\tikzset{corner west below/.code=\tikz@lib@place@handle@{#1}{corner north west}{0}{-1}{corner south west}{1}}
\tikzset{corner east above/.code =\tikz@lib@place@handle@{#1}{corner south east}{0}{1}{corner north east}{1}}
\tikzset{corner east below/.code=\tikz@lib@place@handle@{#1}{corner north east}{0}{-1}{corner south east}{1}}

\tikzset{north left/.code =\tikz@lib@place@handle@{#1}{north east}{-1}{0}{north west}{1}}
\tikzset{north right/.code=\tikz@lib@place@handle@{#1}{north west}{1}{0}{north east}{1}}
\tikzset{south left/.code =\tikz@lib@place@handle@{#1}{south east}{-1}{0}{south west}{1}}
\tikzset{south right/.code=\tikz@lib@place@handle@{#1}{south west}{1}{0}{south east}{1}}

\tikzset{west above/.code =\tikz@lib@place@handle@{#1}{south west}{0}{1}{north west}{1}}
\tikzset{west below/.code=\tikz@lib@place@handle@{#1}{north west}{0}{-1}{south west}{1}}
\tikzset{east above/.code =\tikz@lib@place@handle@{#1}{south east}{0}{1}{north east}{1}}
\tikzset{east below/.code=\tikz@lib@place@handle@{#1}{north east}{0}{-1}{south east}{1}}

\newif\ifqrr@tikz@lib@place@postransform
\tikzset{node distance transformation/.is if=qrr@tikz@lib@place@postransform}
\def\tikz@lib@place@handle@@#1#2#3#4{%
  \pgfutil@in@{of }{#1}%
  \ifpgfutil@in@%
    \tikz@lib@place@of#1\tikz@stop{#4}%
  \else%
    \edef\tikz@lib@place@nums{#1}%
  \fi%
  \ifx\tikz@lib@place@nums\pgfutil@empty%
    % Ok, nothing to do, we have set the anchor and we are happy...
  \else%
    \expandafter\tikz@lib@place@parse@nums\expandafter{\tikz@lib@place@nums}%
    \pgf@x=#2\pgf@x%
    \pgf@y=#3\pgf@y%
    \ifqrr@tikz@lib@place@postransform
      \pgf@pos@transform{\pgf@x}{\pgf@y}% change from original
    \fi
    \edef\tikz@lib@pos@call{\noexpand\pgftransformshift{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  \fi%
}

\def\tikz@lib@place@handle@#1#2#3#4#5#6{%
  \pgfutil@in@{:}{#1}%
  \ifpgfutil@in@
    \tikz@lib@place@handle@qrr@#1\tikz@stop
    \ifx\pgf@temp\pgfutil@empty
      \let\pgf@temp\tikz@node@distance
    \fi
    \pgfmathsetmacro\pgf@tempa{(\pgf@tempa)*#4}%
    \pgfmathsetmacro\pgf@tempb{(\pgf@tempb)*#3}%
    \edef\pgf@marshal{\noexpand\tikz@lib@place@handle@{\pgf@temp}{#2}{\pgf@tempb}{\pgf@tempa}{#5}{#6}}%
    \pgf@marshal
  \else
    \def\tikz@anchor{#2}%
    \let\tikz@do@auto@anchor=\relax%
    \edef\tikz@temp{#1}%
    \def\tikz@lib@place@single@factor{#6}%
    \expandafter\tikz@lib@place@handle@@\expandafter{\tikz@temp}{#3}{#4}{#5}%
  \fi
}
\def\tikz@lib@place@handle@qrr@#1:#2\tikz@stop{%
  \pgfutil@in@{and}{#1}%
  \ifpgfutil@in@
    \tikz@lib@place@handle@qrr@@#1\tikz@stop
  \else
    \tikz@lib@place@handle@qrr@@#1and#1\tikz@stop
  \fi
  \def\pgf@temp{#2}%
}
\def\tikz@lib@place@handle@qrr@@#1and#2\tikz@stop{%
  \def\pgf@tempa{#1}%
  \def\pgf@tempb{#2}%
}
\def\qrr@xyshift@starred#1#2#3{
  \edef\tikz@marshal{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
  \tikz@marshal
  \ifpgfutil@in@
    \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
  \else
    \let#3\tikz@node@distance
  \fi
  \pgfmathparse{(#1)*#3}%
  \ifpgfmathunitsdeclared
    \if#2x%
      \pgftransformshift{\pgfqpoint{\pgfmathresult pt}{0pt}}%
    \else
      \pgftransformshift{\pgfqpoint{0pt}{\pgfmathresult pt}}%
    \fi
  \else
    \ifx#2x
      \pgf@process{\pgfqpointxy{\pgfmathresult}{0}}%
    \else
      \pgf@process{\pgfqpointxy{0}{\pgfmathresult}}%
    \fi
    \pgftransformshift{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \fi}
\tikzset{
  xshift*/.code=\qrr@xyshift@starred{#1}x\pgf@tempb,
  yshift*/.code=\qrr@xyshift@starred{#1}y\pgf@tempa,
}

\def\pgfutil@firstofmany#1#2\pgf@stop{#1}
\def\pgfutil@secondofmany#1#2\pgf@stop{#2}
\def\tikz@lib@place@of@#1#2#3{%
  \def\pgf@tempa{fit bounding box}%
  \edef\pgf@temp{\expandafter\pgfutil@firstofmany#2\pgf@stop}
  \if\pgf@temp(%
    \tikz@lib@place@fit@scan{#2}{0}%
  \else\if\pgf@temp|
      \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{1}%
    \else\ifx\pgf@temp\tikz@activebar
        \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{1}%
      \else\if\pgf@temp-
          \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{2}%
        \else\if\pgf@temp+
            \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{3}%
          \else
            \def\pgf@tempa{#2}%
          \fi
        \fi
      \fi
    \fi
  \fi
  \expandafter\tikz@scan@one@point\expandafter\tikz@lib@place@remember\expandafter(\pgf@tempa)%
  \iftikz@shapeborder%
    % Ok, this is relative to a border.
    \iftikz@lib@ignore@size%
      \edef\tikz@node@at{\noexpand\pgfpointanchor{\tikz@shapeborder@name}{center}}%
      \def\tikz@anchor{center}%
    \else%
      \edef\tikz@node@at{\noexpand\pgfpointanchor{\tikz@shapeborder@name}{#3}}%
    \fi%
  \fi%
  \edef\tikz@lib@place@nums{#1}%
}
\def\tikz@lib@place@fit@scan#1#2{
  \pgf@xb=-16000pt\relax%
  \pgf@xa=16000pt\relax%
  \pgf@yb=-16000pt\relax%
  \pgf@ya=16000pt\relax%
  \if\pgfutil@firstofmany#1\pgf@stop(%
    \tikz@lib@fit@scan#1\pgf@stop%
  \else
    \tikz@lib@fit@scan(#1)\pgf@stop
  \fi
  \ifdim\pgf@xa>\pgf@xa
    % shouldn't happen
  \else
     \expandafter\def\csname pgf@sh@ns@fit bounding box\endcsname{rectangle}%
     \expandafter\edef\csname pgf@sh@np@fit bounding box\endcsname{%
       \def\noexpand\southwest{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
       \def\noexpand\northeast{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
     }%
     \expandafter\def\csname pgf@sh@nt@fit bounding box\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
     \expandafter\def\csname pgf@sh@pi@fit bounding box\endcsname{\pgfpictureid}%
     \ifcase#2\relax
     \or % 1 = vertical
       \pgf@y=\pgf@yb%
       \advance\pgf@y by-\pgf@ya%
       \edef\pgf@marshal{\noexpand\tikzset{minimum height={\the\pgf@y-2*(\noexpand\pgfkeysvalueof{/pgf/outer ysep})}}}%
       \pgf@marshal
     \or % 2 = horizontal
       \pgf@x=\pgf@xb%
       \advance\pgf@x by-\pgf@xa%
       \edef\pgf@marshal{\noexpand\tikzset{minimum width={\the\pgf@x-2*(\noexpand\pgfkeysvalueof{/pgf/outer xsep})}}}%
       \pgf@marshal
     \or % 3 = both directions
       \pgf@y=\pgf@yb%
       \advance\pgf@y by-\pgf@ya%
       \pgf@x=\pgf@xb%
       \advance\pgf@x by-\pgf@xa%
       \edef\pgf@marshal{\noexpand\tikzset{minimum height={\the\pgf@y-2*(\noexpand\pgfkeysvalueof{/pgf/outer ysep})},minimum width={\the\pgf@x-2*(\noexpand\pgfkeysvalueof{/pgf/outer xsep})}}}%
       \pgf@marshal
     \fi
  \fi
}
\tikzset{
  fit bounding box/.code={\tikz@lib@place@fit@scan{#1}{0}},
  span vertical/.code={\tikz@lib@place@fit@scan{#1}{1}},
  span horizontal/.code={\tikz@lib@place@fit@scan{#1}{2}},
  span/.code={\tikz@lib@place@fit@scan{#1}{3}}}

\pgfmathdeclarefunction{x_node_dist}{0}{%
  \begingroup
    \edef\pgfmath@temp{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
    \pgfmath@temp\ifpgfutil@in@
      \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
    \else
      \edef\pgfmath@temp{\tikz@node@distance and\tikz@node@distance}%
      \expandafter\tikz@lib@place@handle@qrr@@\pgfmath@temp\tikz@stop
    \fi
    \pgfmathparse{\pgf@tempb}%
    \pgfmath@smuggleone\pgfmathresult
  \endgroup
}
\pgfmathdeclarefunction{y_node_dist}{0}{%
  \begingroup
    \edef\pgfmath@temp{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
    \pgfmath@temp\ifpgfutil@in@
      \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
    \else
      \edef\pgfmath@temp{\tikz@node@distance and\tikz@node@distance}%
      \expandafter\tikz@lib@place@handle@qrr@@\pgfmath@temp\tikz@stop
    \fi
    \pgfmathparse{\pgf@tempa}%
    \pgfmath@smuggleone\pgfmathresult
  \endgroup
}
%\tikzdeclarecoordinatesystem{node distance}{%
%  \tikz@cs@nd#1\tikz@stop}
%\def\tikz@cs@nd#1,#2\tikz@stop{%
%  \def\qrr@xyshift@starred@action##1{\pgftransformshift{##1}}%
%  \qrr@xyshift@starred{#1}x\pgf@tempb
%  \qrr@xyshift@starred{#2}y\pgf@tempa}
\endinput


==> tikzlibraryqrr.arc.code.tex <==
\tikzset{
  arc/ccw/.initial=1,
  arc/large/.initial=0,
  arc ccw/.style={/tikz/arc/ccw=1},
  arc cw/.style={/tikz/arc/ccw=0},
  arc large/.style={/tikz/arc/large=1},
  arc small/.style={/tikz/arc/large=0},
  arc rotation/.initial=0
}
\def\pgf@temp{2.10-cvs}
\ifx\pgfversion\pgf@temp\else
  \let\tikz@timer@arc\tikz@timer@line
\fi
\def\tikz@arcA rc{\pgfutil@ifnextchar t%
  {\tikz@flush@moveto\expandafter\expandafter\expandafter\tikz@arcB@cont\expandafter\pgfutil@gobble\pgfutil@gobble}
  {\tikz@flush@moveto\tikz@arc@cont}}
\def\tikz@arcB@cont{%
  \pgfutil@ifnextchar[\tikz@@do@arcB{
    \advance\tikz@expandcount by -10\relax% go down quickly
    \ifnum\tikz@expandcount<0\relax%
      \def\@next{\tikz@@do@arcB[]}%
    \else%
      \def\@next{\expandafter\tikz@arcB@cont}%
    \fi%
    \@next}}%
\def\tikz@@do@arcB[#1]{%
  \def\tikz@arcB@options{#1}%
  \tikz@do@@arcB}
\def\tikz@do@@arcB{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@do@@arcB}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@do@@arcB}
      {\tikz@scan@one@point\tikz@do@arcB}}}

\def\tikz@do@arcB#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}
  \tikz@make@last@position{#1}%
  \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \iftikz@shapeborder
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%
  \fi
  \begingroup
    \tikzset{every arc/.try}%
    \expandafter\tikzset\expandafter{\tikz@arcB@options}%
    \pgfmathparse{\pgfkeysvalueof{/tikz/x radius}}%
    \let\tikz@arc@x\pgfmathresult
    \ifpgfmathunitsdeclared
      \pgfmathparse{\pgfkeysvalueof{/tikz/y radius}}%
      \let\tikz@arc@y\pgfmathresult
      \ifpgfmathunitsdeclared
        \edef\tikz@arc@x{\tikz@arc@x pt}%
        \edef\tikz@arc@y{\tikz@arc@y pt}%
        \pgfpatharcto{\tikz@arc@x}{\tikz@arc@y}
                     {\pgfkeysvalueof{/tikz/arc rotation}}{\pgfkeysvalueof{/tikz/arc/large}}
                     {\pgfkeysvalueof{/tikz/arc/ccw}}{#1}%
      \else
        \tikzerror{You cannot mix dimensions and dimension values in an arc}%
      \fi
    \else
      \pgfmathparse{\pgfkeysvalueof{/tikz/y radius}}%
      \let\tikz@arc@y\pgfmathresult
      \ifpgfmathunitsdeclared
        \tikzerror{You cannot mix dimensions and dimension values in an arc}%
      \else
        \pgf@process{\pgfpointxy{\tikz@arc@x}{0}}%
        \pgfmathveclen@{\pgf@x}{\pgf@y}%
        \edef\tikz@arc@x{\pgfmathresult pt}%
        \pgf@process{\pgfpointxy{0}{\tikz@arc@y}}%
        \pgfmathveclen@{\pgf@x}{\pgf@y}%
        \edef\tikz@arc@y{\pgfmathresult pt}%
        \pgfpatharcto{\tikz@arc@x}{\tikz@arc@y}
                     {\pgfkeysvalueof{/tikz/arc rotation}}{\pgfkeysvalueof{/tikz/arc/large}}
                     {\pgfkeysvalueof{/tikz/arc/ccw}}{#1}%
      \fi
    \fi
  \endgroup
  \edef\tikz@timer@start@angle{\expandafter\expandafter\expandafter\pgfutil@firstoffour\expandafter\pgfutil@gobble\pgf@marshal}%
  \edef\tikz@timer@end@angle{\expandafter\expandafter\expandafter\pgfutil@secondoffour\expandafter\pgfutil@gobble\pgf@marshal}%
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\def
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikz@timer@zero@axis
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
  \expandafter\expandafter\expandafter\pgfutil@thirdoffour\expandafter\pgfutil@gobble\pgf@marshal}%
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\def
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikz@timer@ninety@axis
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
  \expandafter\expandafter\expandafter\pgfutil@fourthoffour\expandafter\pgfutil@gobble\pgf@marshal}%
  \let\tikz@timer=\tikz@timer@arc
  \tikz@scan@next@command
}
\def\pgfutil@firstoffour#1#2#3#4{#1}
\def\pgfutil@secondoffour#1#2#3#4{#2}
\def\pgfutil@thirdoffour#1#2#3#4{#3}
\def\pgfutil@fourthoffour#1#2#3#4{#4}


==> tikzlibraryqrr.misc.code.tex <==
%% full arc
\pgfset{full arc/.code=%
  \def\pgf@temp{#1}%
  \ifx\pgfutil@empty\pgf@temp
    \let\pgfmath@fullarc@factor\pgfutil@empty
  \else
    \pgfmathsetmacro\pgfmath@fullarc@factor{360/(#1)}%
  \fi,full arc=}
\pgfmathdeclareoperator{R}{full arc}{1}{postfix}{950}
\pgfmathdeclarefunction{full arc}{1}{%
  \begingroup
    \pgfmath@x=#1pt\relax
    \ifx\pgfmath@fullarc@factor\pgfutil@empty\else
      \pgfmath@x\pgfmath@fullarc@factor\pgfmath@x
    \fi
    \pgfmath@returnone\pgfmath@x
  \endgroup}

%% foreach
% http://tex.stackexchange.com/a/126418/16595
\def\pgffor@scanround(#1)#2,{\def\pgffor@value{(#1)#2}\pgffor@scanned}
% http://tex.stackexchange.com/a/126418/16595
\newif\ifqrr@pgf@foreach@no@list
\pgfqkeys{/pgf/foreach}{
  @use/.code args={#1to#2}{%
    \qrr@pgf@foreach@no@listtrue
    \qrr@pgf@foreach@no@list@use\foreachStart{#1}%
    \pgfutil@in@{step}{#2}
    \ifpgfutil@in@
      \qrr@pgf@foreach@no@list@parse@step#2\pgffor@stop
    \else
      \qrr@pgf@foreach@no@list@parse@step#2step1\pgffor@stop
    \fi
    \edef\qrr@pgf@foreach@no@list@list{\foreachStart,\foreachSecond,...,\foreachEnd}},
  use int/.code={%
    \let\qrr@pgf@foreach@no@list@use\pgfmathtruncatemacro
    \pgfkeysalso{/pgf/foreach/@use={#1}}},
  use float/.code={%
    \let\qrr@pgf@foreach@no@list@use\pgfmathsetmacro
    \pgfkeysalso{/pgf/foreach/@use={#1}}}}
\def\qrr@pgf@foreach@no@list@parse@step#1step#2\pgffor@stop{%
  \qrr@pgf@foreach@no@list@use\foreachEnd{#1}%
  \qrr@pgf@foreach@no@list@use\foreachSecond{\foreachStart+#2}}
\def\pgffor@vars{% manually extended, better etoolbox
  \pgfutil@ifnextchar i{\pgffor@@vars@end}{%
    \pgfutil@ifnextchar[{\pgffor@@vars@opt}{%]
      \pgfutil@ifnextchar/{\pgffor@@vars@slash@gobble}{%
         \ifqrr@pgf@foreach@no@list\expandafter\pgfutil@firstoftwo\else
           \expandafter\pgfutil@secondoftwo\fi
         {\qrr@pgf@foreach@no@listfalse\pgffor@macro@list\qrr@pgf@foreach@no@list@list}
         {\pgffor@@vars}}}}}%

%% Handlers
\pgfkeys{/handlers/.pgfmath/.code=\pgfmathparse{#1}\expandafter\pgfkeys@exp@call\expandafter{\pgfmathresult}}
\pgfkeys{/handlers/.pgfmath int/.code=\pgfmathparse{int(#1)}\expandafter\pgfkeys@exp@call\expandafter{\pgfmathresult}}
\pgfkeys{/handlers/.pgfmath strcat/.code=\pgfmathparse{strcat(#1)}\expandafter\pgfkeys@exp@call\expandafter{\pgfmathresult}}

% http://tex.stackexchange.com/a/144187/16595
\pgfkeys{/handlers/.List/.code={%
    \let\pgfkeys@global@temp\pgfutil@empty
    \foreach \pgfkeys@temp in{#1}{
      \ifx\pgfkeys@global@temp\pgfutil@empty
        \global\let\pgfkeys@global@temp\pgfkeys@temp
      \else
        \expandafter\pgfutil@g@addto@macro\expandafter\pgfkeys@global@temp\expandafter
          {\pgfkeys@temp}%
      \fi}%
    \expandafter\pgfkeys@exp@call\expandafter{\pgfkeys@global@temp}}}

%% PGFmath
\pgfmathdeclarefunction{strrepeat}{2}{%
  \begingroup\pgfmathint{#2}\pgfmath@count\pgfmathresult
    \let\pgfmathresult\pgfutil@empty
    \pgfutil@loop\ifnum\pgfmath@count>0\relax
      \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult#1}%
      \advance\pgfmath@count-1\relax
    \pgfutil@repeat\pgfmath@smuggleone\pgfmathresult\endgroup}

\pgfmathdeclarefunction{instr}{2}{%
  \pgfutil@in@{#1}{#2}%
  \ifpgfutil@in@\def\pgfmathresult{1}\else\def\pgfmathresult{0}\fi}

\pgfmathdeclarefunction{strcat}{...}{%
  \begingroup
    \let\pgfmathresult\pgfutil@empty
    \pgfmathstrcat@@#1\pgfmath@stop}
\def\pgfmathstrcat@@#1{%
  \ifx\pgfmath@stop#1%
    \let\pgfmath@next\pgfmathstrcat@@@
  \else
    \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult#1}%
    \let\pgfmath@next\pgfmathstrcat@@
  \fi
  \pgfmath@next}
\def\pgfmathstrcat@@@{\pgfmath@smuggleone\pgfmathresult\endgroup}


% the CVS version swaps the arguments so I define new atan
% functions that have the order of arguments in their name
\csname pgfmathatan2@\endcsname{0}{1}
\ifdim\pgfmathresult pt=0pt % atan2(y, x)
  \pgfmathdeclarefunction{atanXY}{2}{\csname pgfmathatan2@\endcsname{#2}{#1}}
  \pgfmathdeclarefunction{atanYX}{2}{\csname pgfmathatan2@\endcsname{#1}{#2}}
\else                       % atan2(x, y)
  \pgfmathdeclarefunction{atanXY}{2}{\csname pgfmathatan2@\endcsname{#1}{#2}}
  \pgfmathdeclarefunction{atanYX}{2}{\csname pgfmathatan2@\endcsname{#2}{#1}}
\fi

%% http://tex.stackexchange.com/a/141333/16595
\let\tikz@auto@anchor@orig      \tikz@auto@anchor
\let\tikz@auto@anchor@prime@orig\tikz@auto@anchor@prime
\tikzset{
  Auto/.code=\pgfkeysalso{/tikz/auto=#1}%
    \let\tikz@auto@anchor      \tikz@Auto@anchor
    \let\tikz@auto@anchor@prime\tikz@Auto@anchor@prime,
  auto/.prefix code=\let\tikz@auto@anchor      \tikz@auto@anchor@orig
                    \let\tikz@auto@anchor@prime\tikz@auto@anchor@prime@orig}
\def\tikz@Auto@anchor{%
  \pgfmathatanXY@{\pgf@sys@tonumber\pgf@x}{\pgf@sys@tonumber\pgf@y}%
  \pgfutil@tempdima=\pgfmathresult pt\relax
  \advance\pgfutil@tempdima-90pt\relax
  \edef\tikz@anchor{\pgf@sys@tonumber\pgfutil@tempdima}}
\def\tikz@Auto@anchor@prime{%
  \pgfmathatanXY@{\pgf@sys@tonumber\pgf@x}{\pgf@sys@tonumber\pgf@y}%
  \pgfutil@tempdima=\pgfmathresult pt\relax
  \advance\pgfutil@tempdima90pt\relax
  \edef\tikz@anchor{\pgf@sys@tonumber\pgfutil@tempdima}}

%% http://tex.stackexchange.com/a/132939/16595
\tikzset{
  @edges through/.code={{{% three braces to protect \pgfeov
    \pgfutil@ifnextchar[{\pgfkeysvalueof{/tikz/@@edges through/.@cmd}}
                        {\pgfkeysvalueof{/tikz/@@edges through/.@cmd}[]}#1\pgfeov}}},
  @@edges through/.style args={[#1]#2}{/tikz/insert path={edge[#1] (#2) (#2)}},
  edges through/.style={/tikz/@edges through/.list={#1}}}
\tikzset{
  @edges to/.code={{{% three braces to protect \pgfeov
    \pgfutil@ifnextchar[{\pgfkeysvalueof{/tikz/@@edges to/.@cmd}}
                        {\pgfkeysvalueof{/tikz/@@edges to/.@cmd}[]}#1\pgfeov}}},
  @@edges to/.style args={[#1]#2}{/tikz/insert path={edge[#1] (#2)}},
  edges to/.style={/tikz/@edges to/.list={#1}}}
\tikzset{
  @tos to/.code={{{% three braces to protect \pgfeov
    \pgfutil@ifnextchar[{\pgfkeysvalueof{/tikz/@@tos to/.@cmd}}
                        {\pgfkeysvalueof{/tikz/@@tos to/.@cmd}[]}#1\pgfeov}}},
  @@tos to/.style args={[#1]#2}{/tikz/insert path={to[#1] (#2)}},
  tos to/.style={/tikz/@tos to/.list={#1}}}


==> tikzlibraryqrr.shapes.openrectangle.code.tex <==
\usepgflibrary{qrr.shapes.openrectangle}
\endinput


==> tikzlibraryqrr.trans.code.tex <==
\usepgflibrary{qrr.trans}
\tikzset{
  mirror/.code={%
    \pgfutil@in@{--}{#1}%
    \ifpgfutil@in@
      \tikz@trans@mirror#1\@nil
    \else
      \tikz@scan@one@point\pgfqtransformmirror#1\relax
    \fi},
  ymirror/.code={\pgfutil@ifnextchar(\tikz@trans@ymirror@coordinate\tikz@trans@ymirror@simple#1\@nil},
  xmirror/.code={\pgfutil@ifnextchar(\tikz@trans@xmirror@coordinate\tikz@trans@xmirror@simple#1\@nil},
  mirror x/.code={%
    \pgfextract@process\tikz@temp{\tikz@scan@one@point\pgfutil@firstofone#1\relax}%
    \pgftransformmirror{\tikz@temp}{\pgfpointadd{\tikz@temp}{\pgfqpointxy{0}{1}}}},
  mirror y/.code={%
    \pgfextract@process\tikz@temp{\tikz@scan@one@point\pgfutil@firstofone#1\relax}%
    \pgftransformmirror{\tikz@temp}{\pgfpointadd{\tikz@temp}{\pgfqpointxy{1}{0}}}}
}
\def\tikz@trans@mirror#1--#2\@nil{%
  \pgftransformmirror{\tikz@scan@one@point\pgfutil@firstofone#1\relax}
                     {\tikz@scan@one@point\pgfutil@firstofone#2\relax}}
\def\tikz@trans@xmirror@simple#1\@nil{\pgftransformxmirror{#1}}
\def\tikz@trans@ymirror@simple#1\@nil{\pgftransformymirror{#1}}
\def\tikz@trans@xmirror@coordinate#1\@nil{%
  \tikz@scan@one@point\pgfutil@firstofone#1\pgftransformxmirror{+\the\pgf@x}}
\def\tikz@trans@ymirror@coordinate#1\@nil{\tikz@scan@one@point\pgfutil@firstofone#1\pgftransformymirror{+\the\pgf@y}}
\endinput


==> tikzlibraryshapes.qrr.roundedrectangle.code.tex <==
\usepgflibrary{intersections}%
\pgfset{
  rectangle with rounded corners north west radius/.initial=6pt,
  rectangle with rounded corners north east radius/.initial=6pt,
  rectangle with rounded corners south west radius/.initial=6pt,
  rectangle with rounded corners south east radius/.initial=6pt,
  rectangle with rounded corners radius/.style={
    /pgf/rectangle with rounded corners north west radius={#1},
    /pgf/rectangle with rounded corners north east radius={#1},
    /pgf/rectangle with rounded corners south west radius={#1},
    /pgf/rectangle with rounded corners south east radius={#1}}
}%
\newbox\pgfnodepartlowerbox
\pgfdeclareshape{split rectangle with rounded corners}{%
  \nodeparts{text,lower}%
  \savedmacro\splitrectanglewithroundedcornersparameter{%
    \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/inner ysep}}%
    \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/minimum width}}%
    \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/minimum height}}%
    %
    \pgf@xb\wd\pgfnodeparttextbox
    \advance\pgf@xb\ht\pgfnodeparttextbox
    \advance\pgf@xb\dp\pgfnodeparttextbox
    \pgf@yb\wd\pgfnodepartlowerbox
    \advance\pgf@yb\ht\pgfnodepartlowerbox
    \advance\pgf@yb\dp\pgfnodepartlowerbox
    \ifdim\pgf@yb>\pgf@xb
      \pgf@x\pgf@yb
    \else
      \pgf@x\pgf@xb
    \fi
    \pgf@y\pgf@x
    \advance\pgf@x2\pgf@xa
    \advance\pgf@y2\pgf@ya
    \ifdim\pgf@x<\pgf@xc
      \pgf@x\pgf@xc
    \fi
    \ifdim\pgf@y<\pgf@yc
      \pgf@y\pgf@yc
    \fi
    %
    \pgfutil@tempdima.5\pgf@x
    \pgfutil@tempdimb.5\pgf@y
    \edef\halfWidth{\the\pgfutil@tempdima}%
    \edef\halfHeight{\the\pgfutil@tempdimb}%
    \addtosavedmacro\halfWidth
    \addtosavedmacro\halfHeight
    %
    \advance\pgf@x-2\pgf@xa
    \advance\pgf@y-2\pgf@ya
%    \ifdim\pgf@x<\pgf@y
%      \pgf@x\pgf@y
%    \else
%      \pgf@y\pgf@x
%    \fi
    \pgfutil@tempdima\pgf@x
    \pgfutil@tempdimb\pgf@y
    \pgf@y-.5\pgf@y
    \advance\pgf@y\ht\pgfnodeparttextbox
    \pgf@x.5\pgf@x
    \pgfextract@process\centerpoint{}%
    \addtosavedmacro\centerpoint
    %
    \pgf@x\pgfutil@tempdima
    \pgf@y\pgfutil@tempdimb
    \advance\pgf@x-\wd\pgfnodepartlowerbox
    \advance\pgf@y-\ht\pgfnodeparttextbox
    \advance\pgf@y-\dp\pgfnodepartlowerbox
    \pgf@y-\pgf@y
    \pgfextract@process\loweranchor{}%
    \addtosavedmacro\loweranchor
    %
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/outer ysep}}%
    %
    \pgfextract@process\belownorthwest{%
      \pgfpointadd{\centerpoint}{\pgfqpoint{-\halfWidth}{\halfHeight}}%
      \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/rectangle with rounded corners north west radius}}%
      \advance\pgf@y-\pgfutil@tempdima
      \advance\pgf@x-\pgf@xb
    }%
    \addtosavedmacro\belownorthwest
    %
    \pgfextract@process\leftnortheast{%
      \pgfpointadd{\centerpoint}{\pgfqpoint{\halfWidth}{\halfHeight}}%
      \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/rectangle with rounded corners north east radius}}%
      \advance\pgf@x-\pgfutil@tempdima
      \advance\pgf@y\pgf@yb
    }%
    \addtosavedmacro\leftnortheast
    %
    \pgfextract@process\abovesoutheast{%
      \pgfpointadd{\centerpoint}{\pgfqpoint{\halfWidth}{-\halfHeight}}%
      \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/rectangle with rounded corners south east radius}}%
      \advance\pgf@y\pgfutil@tempdima
      \advance\pgf@x\pgf@xb
    }%
    \addtosavedmacro\abovesoutheast
    %
    \pgfextract@process\rightsouthwest{%
      \pgfpointadd{\centerpoint}{\pgfqpoint{-\halfWidth}{-\halfHeight}}%
      \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/rectangle with rounded corners south west radius}}%
      \advance\pgf@x\pgfutil@tempdima
      \advance\pgf@y-\pgf@yb
    }%
    \addtosavedmacro\rightsouthwest
  }%
  \anchor{lower}{\splitrectanglewithroundedcornersparameter\loweranchor}
  \anchor{center}{\splitrectanglewithroundedcornersparameter\centerpoint}
  \anchor{below north west}{\splitrectanglewithroundedcornersparameter\belownorthwest}
  \anchor{left north east}{\splitrectanglewithroundedcornersparameter\leftnortheast}
  \anchor{above south east}{\splitrectanglewithroundedcornersparameter\abovesoutheast}
  \anchor{right south west}{\splitrectanglewithroundedcornersparameter\rightsouthwest}
  \anchor{west}{\splitrectanglewithroundedcornersparameter
    \centerpoint\pgf@ya\pgf@y \belownorthwest\pgf@y\pgf@ya}
  \anchor{east}{\splitrectanglewithroundedcornersparameter
    \centerpoint\pgf@ya\pgf@y \abovesoutheast\pgf@y\pgf@ya}
  \anchor{north}{\splitrectanglewithroundedcornersparameter
    \centerpoint\pgf@xa\pgf@x \leftnortheast\pgf@x\pgf@xa}
  \anchor{south}{\splitrectanglewithroundedcornersparameter
    \centerpoint\pgf@xa\pgf@x \rightsouthwest\pgf@x\pgf@xa}
  \anchor{mid}{\splitrectanglewithroundedcornersparameter\centerpoint\pgfmathsetlength\pgf@y{+.5ex}}
  \anchor{mid west}{\splitrectanglewithroundedcornersparameter\belownorthwest\pgfmathsetlength\pgf@y{+.5ex}}
  \anchor{mid east}{\splitrectanglewithroundedcornersparameter\abovesoutheast\pgfmathsetlength\pgf@y{+.5ex}}
  \anchor{base}{\splitrectanglewithroundedcornersparameter\centerpoint\pgf@y0pt}
  \anchor{base west}{\splitrectanglewithroundedcornersparameter\belownorthwest\pgf@y0pt}
  \anchor{base east}{\splitrectanglewithroundedcornersparameter\abovesoutheast\pgf@y0pt}
  \anchor{north west}{\splitrectanglewithroundedcornersparameter
    \belownorthwest
    \pgf@xa\pgf@x
    \pgf@xb-\pgf@x
    \pgf@ya\pgf@y
    \leftnortheast
    \advance\pgf@xa\pgf@y
    \advance\pgf@xa-\pgf@ya
    \advance\pgf@xb\pgf@xa
    \pgfpointpolar{135}{\pgf@xb}
    \advance\pgf@x\pgf@xa
    \advance\pgf@y\pgf@ya
  }
  \anchor{south west}{\splitrectanglewithroundedcornersparameter
    \rightsouthwest
    \pgf@xa\pgf@x
    \pgf@ya\pgf@y
    \pgf@yb-\pgf@y
    \belownorthwest
    \advance\pgf@ya-\pgf@x
    \advance\pgf@ya\pgf@xa
    \advance\pgf@yb\pgf@ya
    \pgfpointpolar{225}{\pgf@yb}
    \advance\pgf@x\pgf@xa
    \advance\pgf@y\pgf@ya
  }
  \anchor{south east}{\splitrectanglewithroundedcornersparameter
    \abovesoutheast
    \pgf@ya\pgf@y
    \pgf@xb\pgf@x
    \pgf@xa\pgf@x
    \rightsouthwest
    \advance\pgf@xa\pgf@y
    \advance\pgf@xa-\pgf@ya
    \advance\pgf@xb-\pgf@xa
    \pgfpointpolar{315}{\pgf@xb}
    \advance\pgf@x\pgf@xa
    \advance\pgf@y\pgf@ya
  }
  \anchor{north east}{\splitrectanglewithroundedcornersparameter
    \leftnortheast
    \pgf@xa\pgf@x
    \pgf@ya\pgf@y
    \pgf@yb\pgf@y
    \abovesoutheast
    \advance\pgf@ya-\pgf@x
    \advance\pgf@ya\pgf@xa
    \advance\pgf@yb-\pgf@ya
    \pgfpointpolar{45}{\pgf@yb}
    \advance\pgf@x\pgf@xa
    \advance\pgf@y\pgf@ya
  }
  \anchor{right north west}{\splitrectanglewithroundedcornersparameter
    \belownorthwest\pgf@xa\pgf@x\pgf@ya\pgf@y
    \leftnortheast\pgf@xb\pgf@x
    \advance\pgf@xa\pgf@y
    \advance\pgf@xa-\pgf@ya
    \pgf@x\pgf@xa
  }
  \anchor{below north east}{\splitrectanglewithroundedcornersparameter
    \leftnortheast\pgf@xa\pgf@x\pgf@ya\pgf@y
    \abovesoutheast\pgf@yb\pgf@y
    \advance\pgf@ya-\pgf@x
    \advance\pgf@ya\pgf@xa
    \pgf@y\pgf@ya
  }
  \anchor{left south east}{\splitrectanglewithroundedcornersparameter
    \abovesoutheast\pgf@xa\pgf@x\pgf@ya\pgf@y
    \rightsouthwest\pgf@xb\pgf@x
    \advance\pgf@xa\pgf@y
    \advance\pgf@xa-\pgf@ya
    \pgf@x\pgf@xa
  }%
  \anchor{above south west}{\splitrectanglewithroundedcornersparameter
    \rightsouthwest\pgf@xa\pgf@x\pgf@ya\pgf@y
    \belownorthwest\pgf@yb\pgf@y
    \advance\pgf@ya-\pgf@x
    \advance\pgf@ya\pgf@xa
    \pgf@y\pgf@ya
  }%
  \backgroundpath{%
    \splitrectanglewithroundedcornersparameter
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/outer ysep}}%
    \pgfpathmoveto{\pgfpointadd{\belownorthwest}{\pgfqpoint{\pgf@xb}{+0pt}}}%
    \pgfpathlineto{\pgfpointadd{\pgf@sh@reanchor{split rectangle with rounded corners}{above south west}}{\pgfqpoint{\pgf@xb}{+0pt}}}%
    \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/rectangle with rounded corners south west radius}}%
    \pgfpatharcto{\pgfutil@tempdima}{\pgfutil@tempdima}{0}{0}{1}{\pgfpointadd{\rightsouthwest}{\pgfqpoint{+0pt}{\pgf@yb}}}%
    \pgfpathlineto{\pgfpointadd{\pgf@sh@reanchor{split rectangle with rounded corners}{left south east}}{\pgfqpoint{+0pt}{\pgf@yb}}}%
    \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/rectangle with rounded corners south east radius}}%
    \pgfpatharcto{\pgfutil@tempdima}{\pgfutil@tempdima}{0}{0}{1}{\pgfpointadd{\abovesoutheast}{\pgfqpoint{-\pgf@xb}{+0pt}}}%
    \pgfpathlineto{\pgfpointadd{\pgf@sh@reanchor{split rectangle with rounded corners}{below north east}}{\pgfqpoint{-\pgf@xb}{+0pt}}}%
    \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/rectangle with rounded corners north east radius}}%
    \pgfpatharcto{\pgfutil@tempdima}{\pgfutil@tempdima}{0}{0}{1}{\pgfpointadd{\leftnortheast}{\pgfqpoint{+0pt}{-\pgf@yb}}}%
    \pgfpathlineto{\pgfpointadd{\pgf@sh@reanchor{split rectangle with rounded corners}{right north west}}{\pgfqpoint{+0pt}{-\pgf@yb}}}%
    \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/rectangle with rounded corners north west radius}}%
    \pgfpatharcto{\pgfutil@tempdima}{\pgfutil@tempdima}{0}{0}{1}{\pgfpointadd{\belownorthwest}{\pgfqpoint{\pgf@xb}{+0pt}}}%
    \pgfpathclose
    \loweranchor
    \pgf@xa\pgf@x
    \advance\pgf@y-\dp\pgfnodepartlowerbox
    \pgfpathmoveto{\pgfqpoint{+0pt}{\pgf@y}}%
    \advance\pgf@xa\wd\pgfnodepartlowerbox
    \pgfpathlineto{\pgfqpoint{\pgf@xa}{\ht\pgfnodeparttextbox}}%
  }%
  \anchorborder{%
    \pgf@xb=\pgf@x
    \pgf@yb=\pgf@y
    \pgf@process{\pgf@sh@reanchor{split rectangle with rounded corners}{south}}%
    \pgf@ya\pgf@y
    \pgf@process{\pgf@sh@reanchor{split rectangle with rounded corners}{west}}%
    \pgf@xa\pgf@x
    \pgf@process{\pgf@sh@reanchor{split rectangle with rounded corners}{north}}%
    \pgf@yc\pgf@y
    \pgf@process{\pgf@sh@reanchor{split rectangle with rounded corners}{east}}%
    \pgf@y\pgf@yc
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgf@xc=.5\pgf@x% x/y is half width/height
    \pgf@yc=.5\pgf@y%
    \advance\pgf@xa by\pgf@xc% xa/ya becomes center
    \advance\pgf@ya by\pgf@yc%
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderrectangle
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}
      {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    }%
    \pgf@process{\pgf@marshal}%
    \advance\pgf@xa by\pgf@x%
    \advance\pgf@ya by\pgf@y%
    %
    \pgfutil@tempdima\pgf@xa
    \pgfutil@tempdimb\pgf@ya
%    \pgf@x\pgf@xa
%    \pgf@y\pgf@ya
    \splitrectanglewithroundedcornersparameter
    \centerpoint
    \pgf@xc\pgf@x
    \pgf@yc\pgf@y
    \ifdim\pgfutil@tempdima>\pgf@xc
      \ifdim\pgfutil@tempdimb>\pgf@yc % north east
        \pgf@lib@sh@qrr@get@radius@and@center0\pgfutil@tempdima\pgfutil@tempdimb
      \else                 % south east
        \pgf@lib@sh@qrr@get@radius@and@center3\pgfutil@tempdima\pgfutil@tempdimb
      \fi
    \else
      \ifdim\pgfutil@tempdimb>\pgf@yc % north west
        \pgf@lib@sh@qrr@get@radius@and@center1\pgfutil@tempdima\pgfutil@tempdimb
      \else                 % south west
        \pgf@lib@sh@qrr@get@radius@and@center2\pgfutil@tempdima\pgfutil@tempdimb
      \fi
    \fi
  }
}
\def\pgf@lib@sh@qrr@get@radius@and@center#1#2#3{%
  \begingroup
    \pgfutil@tempswafalse
    \ifcase#1% north east
      \def\pgf@tempa{1}%
      \leftnortheast
      \pgf@xa\pgf@x
      \pgf@ya\pgf@y
      \pgf@yb\pgf@y
      \abovesoutheast
      \advance\pgf@ya-\pgf@x
      \advance\pgf@ya\pgf@xa
      \advance\pgf@yb-\pgf@ya
      \ifdim#3>\pgf@ya
        \ifdim#2>\pgf@xa
          \pgfutil@tempswatrue
        \fi
      \fi
    \or      % north west
      \def\pgf@tempa{1}%
      \belownorthwest
      \pgf@xa\pgf@x
      \pgf@yb-\pgf@x
      \pgf@ya\pgf@y
      \leftnortheast
      \advance\pgf@xa\pgf@y
      \advance\pgf@xa-\pgf@ya
      \advance\pgf@yb\pgf@xa
      \ifdim#3>\pgf@ya
        \ifdim#2<\pgf@xa
          \pgfutil@tempswatrue
        \fi
      \fi
    \or      % south west
      \def\pgf@tempa{2}%
      \rightsouthwest
      \pgf@xa\pgf@x
      \pgf@ya\pgf@y
      \pgf@yb-\pgf@y
      \belownorthwest
      \advance\pgf@ya-\pgf@x
      \advance\pgf@ya\pgf@xa
      \advance\pgf@yb\pgf@ya
      \ifdim#3<\pgf@ya
        \ifdim#2<\pgf@xa
          \pgfutil@tempswatrue
        \fi
      \fi
    \else    % south east
      \def\pgf@tempa{2}%
      \abovesoutheast
      \pgf@ya\pgf@y
      \pgf@yb\pgf@x
      \pgf@xa\pgf@x
      \rightsouthwest
      \advance\pgf@xa\pgf@y
      \advance\pgf@xa-\pgf@ya
      \advance\pgf@yb-\pgf@xa
      \ifdim#3<\pgf@ya
        \ifdim#2>\pgf@xa
          \pgfutil@tempswatrue
        \fi
      \fi
    \fi
    \pgfinterruptboundingbox
      \ifpgfutil@tempswa
        \pgfintersectionofpaths{
          \pgfpathmoveto{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
          \pgfpathlineto{\pgfqpoint{#2}{#3}}%
        }{%
          \pgfpathcircle{\pgfqpoint{\pgf@xa}{\pgf@ya}}{\pgf@yb}%
        }%
        \pgfpointintersectionsolution{\pgf@tempa}
        \pgftransforminvert
        \pgfpointtransformed{}%
      \else
        \pgf@process{\pgfqpoint{#2}{#3}}%
      \fi
    \endpgfinterruptboundingbox
  \endgroup
}
\endinput

